Certifying Higher-Order Polynomial Interpretations

Higher-order rewriting is a framework in which one can write higher-order programs and study their properties. One such property is termination: the situation that for all inputs, the program eventually halts its execution and produces an output. Several tools have been developed to check whether higher-order rewriting systems are terminating. However, developing such tools is difficult and can be error-prone. In this paper, we present a way of certifying termination proofs of higher-order term rewriting systems. We formalize a specific method, namely the polynomial interpretation method, that is used to prove termination. In addition, we give a program that turns the output of Wanda, a termination analysis tool for higher-order rewriting systems, into a Coq script, so that we can check whether the output is a valid proof of termination.

==> notations.tex <==

\usepackage{amsmath,amssymb,amsfonts,amscd,amsbsy,mathtools}
\usepackage{bussproofs}
\usepackage{bm}

\usepackage{xcolor}
\usepackage{xcolor-material}


\newcommand{\syntaxPurble}[1]{\textcolor{MaterialPurple}{#1}}
\newcommand{\syntaxRed}[1]{\textcolor{MaterialRed}{#1}}
\newcommand{\syntaxGold}[1]{\textcolor{GoogleYellow}{#1}}
\newcommand{\syntaxBlue}[1]{\textcolor{GoogleBlue}{#1}}
\newcommand{\syntaxGreen}[1]{\textcolor{GoogleGreen}{#1}}



\newcommand{\sigFont}[1]{\mathsf{#1}}
\newcommand{\sortFont}[1]{\mathsf{#1}}
\newcommand{\varFont}[1]{#1}
\newcommand{\termFont}[1]{#1}
\newcommand{\csPairFont}[1]{\mathcal{#1}}
\newcommand{\compFont}[1]{\mathsf{#1}}


\newcommand{\consFont}[1]{\mathsf{#1}}
\newcommand{\defFont}[1]{\mathsf{#1}}
\newcommand{\undFont}[1]{\mathsf{#1}}
\newcommand{\metaFont}[1]{\mathtt{#1}}

\newcommand{\nat}{\sortFont{nat}}
\newcommand{\lst}{\sortFont{list}}
\newcommand{\real}{\sortFont{real}}
\newcommand{\bool}{\sortFont{bool}}
\newcommand{\word}{\sortFont{W}}

\newcommand{\cost}{\compFont{c}}
\newcommand{\size}{\compFont{s}}
\newcommand{\leng}{\compFont{l}}
\newcommand{\mmax}{\compFont{m}}

\newcommand{\zero}{\consFont{0}}
\newcommand{\nil}{\consFont{nil}}
\newcommand{\suc}{\consFont{s}}
\newcommand{\cons}{\consFont{cons}}
\newcommand{\true}{\consFont{true}}
\newcommand{\false}{\consFont{false}}

\newcommand{\minus}{\consFont{minus}}
\newcommand{\quot}{\consFont{quot}}

\newcommand{\add}{\defFont{add}}
\newcommand{\double}{\defFont{d}}
\newcommand{\mult}{\defFont{mult}}
\newcommand{\append}{\defFont{append}}
\newcommand{\rev}{\defFont{rev}}
\newcommand{\sumList}{\defFont{sum}}
\newcommand{\acc}{\defFont{acc}}
\newcommand{\lessthan}{\defFont{lessthan}}
\newcommand{\ins}{\defFont{insert}}
\newcommand{\isort}{\defFont{isort}}
\newcommand{\ifThenElse}{\defFont{ifThenElse}}
\newcommand{\start}{\defFont{start}}
\newcommand{\sumUp}{\defFont{SumUp}}

\newcommand{\map}{\defFont{map}}
\newcommand{\foldl}{\defFont{foldl}}
\newcommand{\comp}{\defFont{comp}}
\newcommand{\apply}{\defFont{app}}


\newcommand{\listvar}{q}

\newcommand{\asort}{\iota}
\newcommand{\bsort}{\kappa}
\newcommand{\csort}{\nu}
\newcommand{\atype}{A}
\newcommand{\btype}{B}
\newcommand{\ctype}{C}

\newcommand{\afun}{\defFont{f}}
\newcommand{\bfun}{\defFont{g}}
\newcommand{\cfun}{\defFont{h}}

\newcommand{\funF}{\defFont{F}}
\newcommand{\funG}{\defFont{G}}
\newcommand{\funS}{\defFont{S}}


\newcommand{\adata}{\consFont{c}}
\newcommand{\bdata}{\consFont{b}}
\newcommand{\cdata}{\consFont{a}}

\newcommand{\avar}{x}
\newcommand{\bvar}{y}
\newcommand{\cvar}{z}
\newcommand{\aListVar}{xs}
\newcommand{\bListVar}{ys}
\newcommand{\cListVar}{zs}

\newcommand{\aFuncVar}{F}
\newcommand{\bFuncVar}{G}
\newcommand{\cFuncVar}{H}

\newcommand{\aCtx}{\Gamma}
\newcommand{\bCtx}{\Delta}

\newcommand{\aterm}{s}
\newcommand{\bterm}{t}
\newcommand{\cterm}{u}

\newcommand{\num}[1]{\mathsf{#1}}

\newcommand{\aDom}{\csPairFont{A}}
\newcommand{\bDom}{\csPairFont{B}}
\newcommand{\cDom}{\csPairFont{C}}

\newcommand{\costDom}{\aDom^\cost}
\newcommand{\sizeDom}{\aDom^\size}

\newcommand{\costInt}[1]{\mathcal{C}_{#1}}
\newcommand{\costFInt}[1]{\mathcal{F}^\cost_{#1}}
\newcommand{\sizeInt}[1]{\mathcal{S}_{#1}}




\newcommand{\syntaxSig}{\mathfrak{F}}
\newcommand{\signature}{\Sigma}
\newcommand{\F}{\signature}
\newcommand{\dfdS}{\mathcal{D}}
\newcommand{\ctrS}{\mathcal{C}}
\newcommand{\var}{\mathfrak{X}}
\newcommand{\terms}{\mathfrak{T}(\syntaxSig,\var)}
\newcommand{\termsfo}{T_{fo}(\signature,\var)}
\newcommand{\termsfospecial}[1]{T_{fo}(#1,\var)}
\newcommand{\gTerms}{T(\signature)}
\newcommand{\dataTerms}{T(\ctrS)}
\newcommand{\vars}[1]{\mathtt{vars}(#1)}
\newcommand{\fvars}[1]{\mathtt{fv}(#1)}

\newcommand{\sortset}{\b{B}}
\newcommand{\simpletypeset}{\mathbb{T}_\sortset}

\newcommand{\rules}{\mathcal{R}}
\newcommand{\Nat}{\mathbb{N}}
\newcommand{\NatSizeSet}[1]{\Nat^{\typecount{#1}}}
\newcommand{\wm}[1]{\mathrel{\mathcal{WM}_{#1}}}
\newcommand{\trs}{{(\signature,\rules)}}

\newcommand{\arrz}{\to}
\newcommand{\arrzT}{\mathrel{\to^{*}}}
\newcommand{\trsNF}[1]{#1\!\!\downarrow}


\newcommand{\interpret}[1]{\llbracket #1\rrbracket}
\newcommand{\typeinterpret}[1]{\llparenthesis #1 \rrparenthesis}
\newcommand{\sigInt}{\mathcal{J}}

\newcommand{\typecount}[1]{K[#1]}
\newcommand{\sortinterpret}[1]{A_{#1}}

\newcommand{\wmatypes}{\overrightarrow{\typeinterpret{\atype}}}
\newcommand{\weakset}{\text{wm}}
\newcommand{\SM}{\mathcal{M}}
\newcommand{\SMA}{\mathcal{A}_{\SM}}
\newcommand{\ainterpret}[1]{\llbracket#1\rrbracket_{\alpha, \funcinterpret{}}}
\newcommand{\funcinterpret}[1]{\mathcal{J}_{#1}}
\newcommand{\varinterpret}{\alpha}

\newcommand{\sortgr}[1]{>_{#1}}
\newcommand{\sortgeq}[1]{\geq_{#1}}
\newcommand{\typegr}[1]{\sqsupset_{#1}}
\newcommand{\typegeq}[1]{\sqsupseteq_{#1}}
\newcommand{\makesm}[1]{\mathit{MakeSM}_{#1}}

\newcommand{\nul}[1]{\mathtt{0}_{#1}}
\newcommand{\costof}[1]{\mathtt{costof}_{#1}}
\newcommand{\addcost}[1]{\mathtt{addc}_{#1}}


\newcommand{\costGt}{>}
\newcommand{\costGe}{\geq}
\newcommand{\sizeGe}{\sqsupseteq}
\newcommand{\cartGt}{\succ}
\newcommand{\cartGe}{\succcurlyeq}

\newcommand{\bigpair}[1]{\left\langle #1 \right\rangle}
\newcommand{\pair}[1]{\langle #1 \rangle}

\newcommand{\tuple}[1]{\bm{#1}}
\NewDocumentCommand{\typeVec}{m o}{
    \IfValueTF{#2}{
        {}^{#2}\bm{#1}
    }{
        \bm{#1}
    }
}


\newcommand{\fatlambda}{\lambda\!\!\!\lambda}

\newcommand{\app}{\,}
\newcommand{\semApp}{\cdot}

\newcommand{\costWrapper}[1]{\left(#1\right)}

\newcommand{\dom}{\metaFont{dom}}

\newcommand{\unitSet}{\metaFont{unit}}
\newcommand{\unit}{\metaFont{u}}

\newcommand{\hasType}{\mathbin{:}}

\NewDocumentCommand{\irc}{o}{
    \IfValueTF{#1}{
        \metaFont{irc}_{\rules_{#1}}
    }{
        \metaFont{irc}_{\rules}
    }
}
\newcommand{\fpTime}{\ensuremath{\mathtt{FPTIME}}}
\newcommand{\bff}{\ensuremath{\mathtt{BFF}}}
\newcommand{\sfSymbol}{\defFont{S}_f}
\newcommand{\rulesExtd}{\rules_{\funF, f, \funG}}

\newcommand{\subtermR}{\unrhd}
\newcommand{\pSubtermR}{\rhd}

\newcommand{\asub}{\gamma}
\newcommand{\bsub}{\delta}

\newcommand{\dht}[1]{\metaFont{dh}_\rules(#1)}
\newcommand{\ar}{\metaFont{typeOf}}
\newcommand{\lvl}[1]{\metaFont{lvl}(#1)}

\newcommand{\arrtype}{\Rightarrow}
\newcommand{\arrfunc}{\longrightarrow}
\newcommand{\arrfuncwm}{\rightarrow_{\text{wm}}}
\newcommand{\intKey}{\funcinterpret{\sortset/\Nat}}

\newcommand{\bigO}[1]{\mathcal{O}\left( #1 \right)}
\newcommand{\bigTheta}[1]{\Theta\left( #1 \right)}

\newcommand{\deividTODO}[1]{\todo[fancyline]{\textbf{Deivid:}\newline#1}}
\newcommand{\warning}[1]{\syntaxRed{#1}}
\newcommand{\deivid}[1]{\syntaxGreen{#1}}

\newcommand{\defeq}{\coloneqq}

\newcommand{\subTm}[2]{#1[#2]}

\newcommand{\emptycon}{\bullet}
\newcommand{\extendcon}[2]{#1 ,, #2}


\newcommand{\pol}[1]{\consFont{Pol}(#1)}
\newcommand{\polTy}[2]{\consFont{Pol}^{#2}(#1)}

\newcommand{\semTy}[1]{\llbracket #1 \rrbracket}
\newcommand{\semCon}[1]{\llbracket #1 \rrbracket}
\newcommand{\semPoly}[1]{\llbracket #1 \rrbracket}
\newcommand{\semTm}[1]{\llbracket #1 \rrbracket}
\newcommand{\minEl}[1]{\bot_{#1}}
\newcommand{\lvf}[1]{\consFont{lvf}_{#1}}
\newcommand{\plusTyNat}[1]{\consFont{PlusTyNat}_{#1}}
\newcommand{\plusTy}[1]{\consFont{PlusTy}_{#1}}
\newcommand{\slvf}[1]{\consFont{slvf}_{#1}}
\newcommand{\interpretApp}[2]{\consFont{App}(#1, #2)}
